A Proof System with Names for Modal Mu-calculus

Fixpoints are an important ingredient in semantics, abstract interpretation and program logics. Their addition to a logic can add considerable expressive power. One general issue is how to define proof systems for such logics. Here we examine proof systems for modal logic with fixpoints. We present a tableau proof system for checking validity of formulas which uses names to keep track of unfoldings of fixpoint variables as devised by Jungteerapanich.

==> eptcsdata.tex <==
\providecommand{\firstpage}{18}
\providecommand{\publicationstatus}{A. Banerjee, O. Danvy, K.-G. Doh, J. Hatcliff (Eds):\\
David A. Schmidt's 60th Birthday Festschrift\\
EPTCS 129, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.129.2}{10.4204/EPTCS.129.2}}

